Simulation of DAMPE silicon microstrip detectors in the $\rm Allpix^{2}$ framework

Silicon strip detectors have been widely utilized in space experiments for gamma-ray and cosmic-ray detections thanks to their high spatial resolution and stable performance. For a silicon micro-strip detector, the Monte Carlo simulation is recognized as a practical and cost-effective approach to verify the detector performance. In this study, a technique for the simulation of the silicon micro-strip detector with the $\rm Allpix^{2}$ framework is developed. By incorporating the electric field into the particle transport simulation based on Geant4, this framework could precisely emulate the carrier drift in the silicon micro-strip detector. The simulation results are validated using the beam test data as well as the flight data of the DAMPE experiment, which suggests that the $\rm Allpix^{2}$ framework is a powerful tool to obtain the performance of the silicon micro-strip detector.

==> revision.tex <==
Reviewer #1: 

-References [6], [7], [12]: Incomplete references. Can't find them with provided information to follow-through to verify relevance.
-Are references [12] and [15] supposed to be referring to the same publication?

References 6 and 7 are conference papers, and we have updated the BibTeX and reference display style. Reference 12, originally a software citation, has been updated to reference the article, in line with reference 15.



-Line 22: "charge sharing algorithm in [8] due"
done.



-Fig 1: Please make use of different line types such as solid, dotted, and dashed, or dot-dash. I can't easily tell the difference between the GEANT4 and on-orbit data.

In Figure 1, for the total ADC count, we used two different markers to distinguish between GEANT4 and on-orbit data. For cluster size, we used two different line types.



-Line 59: Change "construction" to "design"
done.



-Lines 62-63: The STK, shown in Fig. 2, is a sub-detector of DAMPE [18] which primarily measures the track and charge of an incident particle.

We have rewritten the relevant sentences according to your suggestion.



-Fig 5 caption. Rephrase second sentence into two sentences without commas: "Only the range of 90 um which exhibits the greatest change in electric field is presented here. The unit of electric field strength is V/m."

We have rewritten the relevant sentences according to your suggestion.



-Line 45: Change "causing" to "requiring".
done.

Line 169: Change "capacitance" to "capacitors". I assume that you are referring to Fig 3 in [8], which shows component capacitors.
done.



-Line 173: Change "capacitor" to "capacitors"
done.



-Lines 182-185: I recommend the following wording, provided I understand what the authors are trying to say here:
As Allpix2 can only provide the generated charge signal of each strip, we must incorporate a noise component as determined with on-orbit data into the corresponding simulated readout strips, and then independently handle the remaining digitization process based on the specific characteristics of our detector.

Thanks, We have rewritten the relevant sentences according to your suggestion.


-Fig 9: I don't think that the left-hand half of the figure is useful. I recommend deleting it, leaving only the right-hand half with the 1D histogram. It is not clear what the point of the 2D histogram is, since it very featureless. Perhaps the point of that 2D histogram may be made with words: "There is no pattern to the location of noisy channels."

We have removed the left-side figure and retained only the right-side image.



-Line 250: Delete "following cluster features:"
done.



-Fig 16 caption: "The responses of protons (left) and helium (right) hitting"
done.

The modified sections have been highlighted in blue within the article. Thank you for your suggestion once again.
